Probabilistic Control of Heterogeneous Swarms Subject to Graph Temporal Logic Specifications: A Decentralized and Scalable Approach

We develop a probabilistic control algorithm, $\texttt{GTLProCo}$, for swarms of agents with heterogeneous dynamics and objectives, subject to high-level task specifications. The resulting algorithm not only achieves decentralized control of the swarm but also significantly improves scalability over state-of-the-art existing algorithms. Specifically, we study a setting in which the agents move along the nodes of a graph, and the high-level task specifications for the swarm are expressed in a recently-proposed language called graph temporal logic (GTL). By constraining the distribution of the swarm over the nodes of the graph, GTL can specify a wide range of properties, including safety, progress, and response. $\texttt{GTLProCo}$, agnostic to the number of agents comprising the swarm, controls the density distribution of the swarm in a decentralized and probabilistic manner. To this end, it synthesizes a time-varying Markov chain modeling the time evolution of the density distribution under the GTL constraints. We first identify a subset of GTL, namely reach-avoid specifications, for which we can reduce the synthesis of such a Markov chain to either linear or semi-definite programs. Then, in the general case, we formulate the synthesis of the Markov chain as a mixed-integer nonlinear program (MINLP). We exploit the structure of the problem to provide an efficient sequential mixed-integer linear programming scheme with trust regions to solve the MINLP. We empirically demonstrate that our sequential scheme is at least three orders of magnitude faster than off-the-shelf MINLP solvers and illustrate the effectiveness of $\texttt{GTLProCo}$ in several swarm scenarios.

==> bil_accuracy.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,1,1}


\begin{axis}[
legend cell align={left},
legend columns=3,
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1)},
  anchor=south west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Number of bins},
xmajorgrids,
xmin=0.25, xmax=104.75,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy of bilinear constraint},
ymajorgrids,
ymin=-5.9070130262079e-08, ymax=1.24047273550366e-06,
ytick style={color=black},
ytick={-2e-07,0,2e-07,4e-07,6e-07,8e-07,1e-06,1.2e-06,1.4e-06},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2,1.4}
]
\path [draw=blue, fill=blue, opacity=0.5]
(axis cs:5,3.51979409663545e-08)
--(axis cs:5,0)
--(axis cs:10,1.38777878078145e-17)
--(axis cs:15,1.38777878078145e-17)
--(axis cs:20,1.38777878078145e-17)
--(axis cs:25,1.2490009027033e-16)
--(axis cs:30,1.73472347597681e-17)
--(axis cs:35,9.9475983006414e-14)
--(axis cs:40,2.70006239588838e-13)
--(axis cs:45,3.12250225675825e-16)
--(axis cs:50,2.1316282072803e-14)
--(axis cs:55,7.105427357601e-14)
--(axis cs:60,3.08780778723872e-16)
--(axis cs:65,3.76585915229377e-13)
--(axis cs:70,3.21964677141295e-15)
--(axis cs:75,8.54871728961371e-15)
--(axis cs:80,6.66133814775094e-16)
--(axis cs:85,1.70530273929659e-11)
--(axis cs:90,4.57966997657877e-16)
--(axis cs:95,3.58639340447553e-10)
--(axis cs:100,1.38634659307968e-11)
--(axis cs:100,2.58162603677252e-07)
--(axis cs:100,2.58162603677252e-07)
--(axis cs:95,3.87152823422864e-07)
--(axis cs:90,4.17698547643293e-07)
--(axis cs:85,3.99809907355823e-07)
--(axis cs:80,3.47378166260805e-07)
--(axis cs:75,4.7825025673312e-07)
--(axis cs:70,3.02981417132219e-07)
--(axis cs:65,5.0500622746743e-07)
--(axis cs:60,4.38246786705883e-07)
--(axis cs:55,5.80222772644314e-07)
--(axis cs:50,7.05517631062206e-07)
--(axis cs:45,5.85493785973419e-07)
--(axis cs:40,3.50843325431737e-07)
--(axis cs:35,4.66660604784314e-07)
--(axis cs:30,5.4318926166212e-08)
--(axis cs:25,2.97246252410578e-07)
--(axis cs:20,3.75810419181088e-07)
--(axis cs:15,9.94961443131091e-08)
--(axis cs:10,2.74532898567441e-08)
--(axis cs:5,3.51979409663545e-08)
--cycle;

\path [draw=green!50.1960784313725!black, fill=green!50.1960784313725!black, opacity=0.5]
(axis cs:5,2.33842298007347e-07)
--(axis cs:5,2.98483160132701e-08)
--(axis cs:10,7.13774552241198e-08)
--(axis cs:15,8.52324744463062e-08)
--(axis cs:20,1.45057253021452e-07)
--(axis cs:25,1.40648975313629e-07)
--(axis cs:30,1.92876002418618e-07)
--(axis cs:35,4.76056553300996e-08)
--(axis cs:40,2.22367496088068e-07)
--(axis cs:45,3.47035166176896e-07)
--(axis cs:50,3.88358204743906e-07)
--(axis cs:55,3.51433544220554e-07)
--(axis cs:60,3.91706157418116e-07)
--(axis cs:65,5.67333178236055e-07)
--(axis cs:70,4.76279673286626e-07)
--(axis cs:75,8.61987766033467e-07)
--(axis cs:80,6.7842250658821e-07)
--(axis cs:85,8.70002807511437e-07)
--(axis cs:90,8.51222166106322e-07)
--(axis cs:95,8.5935438625534e-07)
--(axis cs:95,8.5935438625534e-07)
--(axis cs:95,8.5935438625534e-07)
--(axis cs:90,9.95474450760092e-07)
--(axis cs:85,1.01722796699358e-06)
--(axis cs:80,9.22658332470558e-07)
--(axis cs:75,1.18140260524158e-06)
--(axis cs:70,8.57333279756164e-07)
--(axis cs:65,9.08774401734594e-07)
--(axis cs:60,8.35980373506906e-07)
--(axis cs:55,8.62941618425147e-07)
--(axis cs:50,8.56664555445891e-07)
--(axis cs:45,1.04792557291441e-06)
--(axis cs:40,7.89402094815504e-07)
--(axis cs:35,8.52950211281527e-07)
--(axis cs:30,8.00236316962089e-07)
--(axis cs:25,6.90396594736297e-07)
--(axis cs:20,6.58642822693917e-07)
--(axis cs:15,6.48373608262732e-07)
--(axis cs:10,5.05492285112859e-07)
--(axis cs:5,2.33842298007347e-07)
--cycle;

\path [draw=color0, fill=color0, opacity=0.5]
(axis cs:5,7.46087722844579e-08)
--(axis cs:5,2.53257456600455e-08)
--(axis cs:10,3.00000078667928e-08)
--(axis cs:15,4.98402058096703e-08)
--(axis cs:20,6.99098198081449e-08)
--(axis cs:25,6.99799302741888e-08)
--(axis cs:30,1.08203517902583e-07)
--(axis cs:30,1.08203517902583e-07)
--(axis cs:30,1.08203517902583e-07)
--(axis cs:25,4.36910632924615e-07)
--(axis cs:20,4.45751569951104e-07)
--(axis cs:15,4.63764225116229e-07)
--(axis cs:10,2.89896903081584e-07)
--(axis cs:5,7.46087722844579e-08)
--cycle;

\path [draw=white!50.1960784313725!black, fill=white!50.1960784313725!black, opacity=0.5]
(axis cs:5,1.46722546686323e-08)
--(axis cs:5,0)
--(axis cs:5,1.46722546686323e-08)
--(axis cs:5,1.46722546686323e-08)
--cycle;

\addplot [thick, blue, mark=*, mark size=2.5, mark options={solid}]
table {%
5 1.16437697914029e-08
10 8.35481775499081e-09
15 3.28025754312705e-08
20 1.20247830828063e-07
25 8.33789008249791e-08
30 1.61912381026891e-08
35 1.98796520245979e-07
40 1.10044076943872e-07
45 2.51166169392206e-07
50 3.45627389773499e-07
55 2.69013964492894e-07
60 1.76175215288368e-07
65 2.3370847140004e-07
70 1.30681159692548e-07
75 1.77022941562008e-07
80 1.55819889684824e-07
85 1.7561032411139e-07
90 1.66676926081737e-07
95 1.90916635234815e-07
100 1.04820524363374e-07
};
\addlegendentry{GTLProco}
\addplot [thick, green!50.1960784313725!black, mark=asterisk, mark size=2.5, mark options={solid}]
table {%
5 1.02290918314873e-07
10 2.5587002009872e-07
15 3.41857260734504e-07
20 4.01850037857684e-07
25 3.91741372458149e-07
30 4.96556159690353e-07
35 4.50277933305814e-07
40 5.05884795451786e-07
45 6.97480369545655e-07
50 6.22511380094898e-07
55 6.07187581322851e-07
60 6.13843265462511e-07
65 7.38053789985325e-07
70 6.67206969970506e-07
75 1.02060726588464e-06
80 8.0925263091277e-07
85 9.43615387252507e-07
90 9.23348308433207e-07
95 8.5935438625534e-07
};
\addlegendentry{Gurobi_MINLP}
\addplot [thick, color0, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
5 4.99672589722517e-08
10 1.26082197601796e-07
15 2.19302350609817e-07
20 2.49064695108554e-07
25 2.33647629993561e-07
30 1.08203517902583e-07
};
\addlegendentry{SCIP}
\addplot [thick, white!50.1960784313725!black, mark=triangle*, mark size=2.5, mark options={solid}]
table {%
5 4.40769853717512e-09
};
\addlegendentry{couenne}
\end{axis}

\end{tikzpicture}

